Linear lambda Calculus with Explicit Substitutions as Proof-Search in Deep Inference

SBV is a deep inference system that extends the set of logical operators of multiplicative linear logic with the non commutative operator Seq. We introduce the logical system SBVr which extends SBV by adding a self-dual atom-renaming operator to it. We prove that the cut elimination holds on SBVr. SBVr and its cut free subsystem BVr are complete and sound with respect to linear lambda calculus with explicit substitutions. Under any strategy, a sequence of evaluation steps of any linear lambda-term M becomes a process of proof-search in SBVr (BVr) once M is mapped into a formula of SBVr. Completeness and soundness follow from simulating linear beta-reduction with explicit substitutions as processes. The role of the new renaming operator of SBVr is to rename channel-names on-demand. This simulates the substitution that occurs in a beta-reduction. Despite SBVr is a minimal extension of SBV its proof-search can compute all boolean functions, as linear lambda-calculus with explicit substitutions can compute all boolean functions as well. So, proof search of SBVr and BVr is at least ptime-complete.

==> BV2-substitution.tex <==
\begin{align*}
 \atmb\subst{\atma}{\atmb} & = \atma
 \\
 \atmc\subst{\atma}{\atmb} & = \atmc
 \\
 \vlfo{\atmb}{\strR}\subst{\atma}{\atmb} & = \strR
 \\
 \vlfo{\atmc}{\strR}\subst{\atma}{\atmb} & =
    \vlfo{\atmc}{\strR\subst{\atma}{\atmb}}
 \\
%  \vlsbr<\strR;\strT>\subst{\atma}{\atmb} & =\
%     \vlsbr<\strR\subst{\atma}{\atmb};\strT\subst{\atma}{\atmb}>
%  \\
%  \vlsbr(\strR,\strT)\subst{\atma}{\atmb} & =\
%     \vlsbr(\strR\subst{\atma}{\atmb};\strT\subst{\atma}{\atmb})
%  \\
%  \vlsbr[\strR,\strT]\subst{\atma}{\atmb} & =\
%     \vlsbr[\strR\subst{\atma}{\atmb},\strT\subst{\atma}{\atmb}]
%  \\
\end{align*}
 


==> BV2Min-system.tex <==
\begin{tabular}{ccc}
$\vlinf{\bvtatidrule}{}{\vlsbr[<[\atma,\natma];\strR>,\strT]}
                       {\vlsbr[\strR,\strT]}$
&
&
$\vlinf{\bvtatiurule}{}{\vlsbr[\strR,\strT]}
                       {\vlsbr(<[\atma,\natma];\strR>,\strT)}$
\end{tabular} 


==> BV2Min.tex <==
\section{The restriction $\BVMin$ of $\BVT$}
\label{section:The restriction BVMin of BVT}
We introduce a restriction $\BVMin$ of $\BVT$, and, correspondingly, 
$\SBVMin$ of $\SBVT$, that enjoys cut elimination and which is correct \wrt\
\llcxLamCalc. We remark that $\BVT$ is not correct because it proves
structures which are by no means representation of any \llcxLamTerm.
So, proving structures in $\BVMin$ is exactly as computing in \llcxLamCalc.
The relevance of computing inside $\BV$ is connected to the cut elimination we
can prove in its completely symmetric version $\SBVMin$. The idea is to search
for efficient cut elimination strategies, analogous to the one in 
\cite{BrusGuglGundPari:09:A-Quasip:fk}.

%%%%%%%%%%%
\begin{figure}[ht]
\begin{center}
\fbox{
        \begin{minipage}{.9\textwidth}
        \begin{center}
        %%%%%%%%%%%%%
        \input{BV2Min-system}
        %%%%%%%%%%%%%
        \end{center}
        \end{minipage}
    }%\fbox
\end{center}
\caption{The set of rules of $\BVMin$.}
    \label{fig:BV2Min-system}
\end{figure}


\paragraph{Legal structures or, simply, structures.}
The set $\strSET$ of \dfn{legal structures} contains \dfn{freely generated
structures} subject to specific constraints. We say that a freely generated
structure $\strS$ is \dfn{legal} iff, every of its atoms occur at most twice in
$\strS$. We add one to the count of the occurrences of a given $\atma$ whenever
we meet $\atma$ or $\natma$. 

For example, $\atma$ and, $\atmb$ occur once in
$\vlfo{\atma}{{\vlsbr[\natma.\atmb]}}$. So, the bound occurrence of $\atma$. We
have one occurrence of $\atma$ in ${\vlsbr[\natma;\vlfo{\atma}{\natma}]}$
because it is $\alpha$-equivalent to ${\vlsbr[\natma;\vlfo{\atmb}{\natmb}]}$.
Also $\vlanbrl \vlfo{\atma}{{\vlsbr[\atma;\natma]}} \vlse
\vlfo{\atma}{{\vlsbr(\atma;\natma)}} \vlse \natma \vlanbrr$ is legal, because
$\alpha$-equivalent to $\vlanbrl \vlfo{\atmb}{{\vlsbr[\atmb;\natmb]}} \vlse
\vlfo{\atmc}{{\vlsbr(\atmc;\natmc)}} \vlse \natma \vlanbrr$. Finally,
${\vlsbr(\atma;\vlfo{\atmb}{\vlanbrl \atma \vlse \natma \vlanbrr})}$ is not
legal because $\atma$ occurs three times. We range over $\strSET$ by $\strS,
\strR, \strT, \strU, \strV$.


==> SBV2+-structure-equivalences.tex <==
  \begin{center}
%     \vspace{-1.5\baselineskip}
    \begin{tabular}{cc}
      \begin{minipage}{.45\textwidth}
       \begin{center}
        \smalltitle{\textbf{Negation}}%
        {%do not erase
         \begin{align}
           \nonumber
           \vlne{{\vlsbr[\strR\vlpl\strT]}} &
           \approx {\vlsbr[\vlne{\strR}\vlpl\vlne{\strT}]}
         \end{align}
        }%do not erase

%         \smalltitle{\textbf{Binder}}%
%         {%do not erase
%                 \begin{align*}
%                   \strR & \approx \vlfo{\atma}{\strR\subst{\atma}{\atmb}} \\
%                   \atmb\subst{\atma}{\atmb} & \approx \atma               \\
%                   \natmb\subst{\atma}{\atmb} & \approx \natma               \\
%                   \atmc\subst{\atma}{\atmb} & \approx\atmc                \\
%                   \natmc\subst{\atma}{\atmb} & \approx\natmc                \\
%                   {\vlsbr[\strR;\strT]}\subst{\atma}{\atmb} &
%                         \approx
%                      {\vlsbr[\strR\subst{\atma}{\atmb};
%                              \strT\subst{\atma}{\atmb}]} \\
%                   {\vlsbr(\strR;\strT)}\subst{\atma}{\atmb} &
%                         \approx
%                      {\vlsbr(\strR\subst{\atma}{\atmb};
%                              \strT\subst{\atma}{\atmb})} \\
%                   {\vlsbr<\strR;\strT>}\subst{\atma}{\atmb} &
%                         \approx
%                      {\vlsbr<\strR\subst{\atma}{\atmb};
%                              \strT\subst{\atma}{\atmb}>} \\
%                   \vlfo{\atmb}{\strR}\subst{\atma}{\atmb} & \approx \strR \\
%                   \vlfo{\atmc}{\strR}\subst{\atma}{\atmb} & \approx
%                        \vlfo{\atmc}{\strR\subst{\atma}{\atmb}}
%                 \end{align*}
%         }%do not erase

%        \end{center}
%       \end{minipage}
%       &
%       \begin{minipage}{.45\textwidth}
%        \begin{center}
%         \vspace{2\baselineskip}
        %%%

%         %%%
%         \smalltitle{\textbf{Contextual Closure}}\\%
%         {%do not erase
%           ${\strS{\vlscn{\strR}}} \approx {\strS{\vlscn{\strT}}}$ if
%           $\strR\approx \strT$
%         \vspace{\baselineskip}          
% %         \vspace{\baselineskip}
%         }%do not erase

        \smalltitle{\textbf{Unit}}%
        {%do not erase
                \begin{align*}
%                   \strR           & \approx{\vlsbr[\strR]}
%                                     \approx{\vlsbr(\strR)}
%                                     \approx{\vlsbr<\strR>}
%                   \\
                  \vlone  & \approx{\vlsbr[\vlzer\vlpl\vlone]} 
%                   \\
%                   \vlone          & \approx{\vlfo{\atma}{\vlone}}
                \end{align*}
        }%do not erase

        \smalltitle{\textbf{Associativity}}%
        {%do not erase
          \begin{align*}
          {\vllutzsyntax
           \vlsbr[[\strR\vlpl\strT]\vlpl\strV]} &
           \approx {\vllutzsyntax
            \vlsbr[\strR\vlpl[\strT\vlpl\strV]]}
        \end{align*}
        }%do not erase

        \smalltitle{\textbf{Commutativity}}%
        {%do not erase
                \begin{align*}
                 {\vlsbr[\strR\vlpl\strT]}  & \approx{\vlsbr[\strT\vlpl\strR]}
                \end{align*}
        }%do not erase


        \smalltitle{\textbf{Distributivity}}%
        {%do not erase
                \begin{align*}
		  {\vlfo{\atma}{\vlsbr[\strR\vlpl\strU]}} & \approx
		  {\vlsbr[{\vlfo{\atma}{\strR}}\vlpl{\vlfo{\atma}{ \strU}}]}
                \end{align*}
        }%do not erase

%         %%%
%         \smalltitle{\textbf{Exchange}}%
%         {%do not erase
%                 \begin{align*}
%                  \vlfo{\atma}{\vlex{\atmb}{\strR}}
%                   & \approx \vlex{\atmb}{\vlfo{\atma}{\strR}}
%                 \end{align*}
%         }%do not erase

       \end{center}
      \end{minipage}
    \end{tabular}
   \vspace{\baselineskip}
  \end{center}


==> SBV2+-system.tex <==
\begin{tabular}{cc}
$\vlinf{\bvtpludrule}{}
        {{\vlsbr[[\strR\vlpl\strU];\strT]}}
        {{\vlsbr[[\strR;\strT]\vlpl[\strU;\strT]]}}$
&
$\vlinf{\bvtpluurule}{}
        {{\vlsbr[(\strR;\strT)\vlpl(\strU;\strT)]}}
        {{\vlsbr([\strR\vlpl\strU];\strT)}}$
\\\\
$\vlinf{\bvtawedrule}{}{\strR}
                       {\vlzer}$
&
$\vlinf{\bvtaweurule}{}{\vlzer}
                       {\strR}$
\end{tabular}

==> SBV2Min-to-LLCXS.tex <==
\section{Soundness of $\SBVMin$} 
\label{section:Soundness of SBVMin} 

We show that $\BVMin$ ``is'' \llcxLamCalc\ in logical form. Namely, every
proof in $\BVMin$ is a $\beta$-reduction with explicit substitutions of
\llcxLamCalc.

\Luca{Da sviluppare \ldots}
